Exploration and Online Transfer with Behavioral Foundation Models

Zero-shot Transfer in Reinforcement Learning (RL) aims to train an agent that can generate optimal policies for any reward function, without additional learning at transfer time, while training only on reward-free trajectories. For their generality over tasks, such models are sometimes called ``Behavioral Foundation Models'' (BFMs). While they have shown strong performances and improvements in recent years, the current framework and algorithms still assume that, during the transfer phase, the agent is informed offline about the reward (the task to solve) through a dataset of state-reward pairs, which it uses to pick the best policy to deploy. However, in practice if the reward is a black-box (e.g. direct user feedback), it is not possible to generate such a dataset: it is necessary to observe the reward through interactions with the environment. In other words, the current framework of offline transfer is not aligned with the traditional RL setting of online learning through trial-and-error, which requires exploration in order to find rewards. This paper proposes to tackle this new online transfer in zero-shot RL, with the key insight that the BFM itself can be used to generate exploration policies. We show that it is possible to frame this online learning problem in terms of a bandit-like exploration-exploitation problem. More precisely, at each step the bandit algorithm recommends a policy, the BFM executes it in the environment, which yields a reward and a new state; we repeat the process until we converge to the optimal policy. In the popular context of linear reward approximation, we derive a formulation inspired by Upper Confidence Bound and show that exploration can be achieved through the minimization of the eigenvalues of an uncertainty matrix. We evaluate qualitatively and quantitatively our framework on a simple environment to validate the concept of our method.

==> _unsed_fig_transfer.tex <==
\begin{figure}
    \centering
    \includegraphics[height=0.08\textheight]{img/exploit/to_solve_cluster.pdf}
    %\hspace*{0.5pt}
    \vrule
    \includegraphics[height=0.08\textheight]{img/exploit/solved_clusters.pdf}
    \includegraphics[height=0.08\textheight]{img/exploit/to_solve_lap.pdf}
    %\hspace*{0.8pt}
    \vrule
    \includegraphics[height=0.08\textheight]{img/exploit/solved_lap.pdf}
    \caption{Performing exploration and exploitation. On the left, we display the task vector $\z_r$ to find. The agent needs to interact with the domain to maximize this reward. We then display the trajectory, every $5$ steps, as the agent explores and eventually exploits. In the background we now show only the linear least squares estimate $\hat{Z}_t$. We can see that the agent's estimation does converge, and it ends up performing the optimal policy.}
    \label{fig:exploit}
\end{figure}

==> _unused_fig_intro.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\textwidth]{img/offline_online_transfer.pdf}
    \caption{Difference between \textit{offline} transfer, as standard in zero-shot RL literature, and the \textit{online} transfer we propose. In offline transfer, a dataset of state-reward pairs enables us to directly compute the optimal task vector, which the Behavior Foundation Model (BFM) uses to execute the optimal policy. However, in practice, we often cannot generate such a dataset, so interactions with the environment are necessary: this is \textit{online} transfer. We propose a framework inspired by the Bandit problem where an Algorithm must \textit{recommend} a task vector for the BFM to execute, and use the reward feedback from the environment to converge to the optimal task vector.
    }
    \label{fig:framework}
\end{figure}

==> fig_intro_old.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/framework.pdf}
    \caption{Framework proposed for exploration with Behavioral Foundation Models (BFM) on a 2D navigation task. In a pre-training phase, the model is trained to solve all tasks encoded by its task encoding $\z \in \sR ^d $ (on the figure we show cluster occupancy features). The model is then frozen for the transfer phase. To obtain an exploration policy, we sequentially pick encoding vectors $Z_t$ that push the agent towards exploration (minimal uncertainty). Our bandit approach means that at each step, we \textit{recommend} a task encoding, and its associated policy is executed (step 2).
    This framework is unchanged if we need to solve a black-box reward revealed at each time-step, $R_{t+1}$, where the recommendation should now converge to the true or encoded reward function.
    }
    \label{fig:framework}
\end{figure}
